Ethical Adversaries: Towards Mitigating Unfairness with Adversarial Machine Learning

Machine learning is being integrated into a growing number of critical systems with far-reaching impacts on society. Unexpected behaviour and unfair decision processes are coming under increasing scrutiny due to this widespread use and its theoretical considerations. Individuals, as well as organisations, notice, test, and criticize unfair results to hold model designers and deployers accountable. We offer a framework that assists these groups in mitigating unfair representations stemming from the training datasets. Our framework relies on two inter-operating adversaries to improve fairness. First, a model is trained with the goal of preventing the guessing of protected attributes' values while limiting utility losses. This first step optimizes the model's parameters for fairness. Second, the framework leverages evasion attacks from adversarial machine learning to generate new examples that will be misclassified. These new examples are then used to retrain and improve the model in the first step. These two steps are iteratively applied until a significant improvement in fairness is obtained. We evaluated our framework on well-studied datasets in the fairness literature -- including COMPAS -- where it can surpass other approaches concerning demographic parity, equality of opportunity and also the model's utility. We also illustrate our findings on the subtle difficulties when mitigating unfairness and highlight how our framework can assist model designers.

==> background.tex <==
%In the following, we introduce the conceptual foundations on which our ethical adversaries framework relies, namely adversarial fairness and evasion attacks.

\subsection{Adversarial machine learning}\label{ss:adv}
Adversarial machine learning aims at finding or creating examples that are problematic for a machine learning model, \textit{e.g.}, \citep{papernot2016,papernot2017,biggio2013evasion}. \citet{biggio2018} synthesised a decade of research in adversarial machine learning.
These techniques follow the same process: probe an existing target machine learning based system to gain information about it, copy an existing example, apply an adversarial technique that will modify the example depending on the desired goal.
Modified examples show an interesting behavior: they remain similar to the original ones while being misclassified by the trained model.
%In particular, adversarial machine learning targets a model under attack and generate adversarial examples based on information retrieved on this model.
Various models can be attacked including support vector machines (SVMs), linear models or even (deep) neural networks (NNs).
%While several work try to understand how adversarial examples are generated on well-known models (such as SVMs, linear models, etc.); 
While adversarial machine learning begins with a model of attackers' possibilities, it also enables the design of defenses against attacks.
In particular, adversarial retraining has been very popular with the emergence of generative adversarial nets (GANs) proposed by \citet{goodfellowGenerativeAdversarialNets2014a}. 
%The idea is to incorporate adversarial examples directly into the training set such that the resulting model becomes less sensitive to them.
%For instance, Goodfellow et al. analysed the problem with Deep Neural Networks\citep{goodfellowGenerativeAdversarialNets2014a, goodfellowExplainingHarnessingAdversarial2014}.
%In particular, they proposed the Generative Adversarial Nets (GANs) architecture which confront Neural Networks to generated adversarial examples directly in the training process to make them more robust to such kind of attacks.
Other approaches to robustify neural networks exist and use existing examples: \textit{e.g.}, \citet{edwards2015} used an adversary to force an encoder-decoder network to learn domain-independent representations~\citep{edwards2015, madrasLearningAdversariallyFair2018, zhangMitigatingUnwantedBiases2018}.

%Recently, adversarial machine learning techniques have been used to test the behavior of safety-critical ML-based systems \citep{pei2017deepxplore,tian2018deeptest,zhang2018deeproad}.

%These techniques question the assumption stating that the distribution of data is stationary. In other words, one assumes the distributions between the training set and the test set are similar (and ideally the same) but this does not necessarily holds.
%For example, spam filters are trained on millions of instances, yet, new spams are crafted by modifying certain words (hence changing the underlying distribution) to be considered as genuine emails.

%\subsection{Adversarial machine learning with fairness constraints}
\subsection{Fair Representations with Neural Networks}
\label{ss:adv-ml}

Several works~\citep{raff2018, adel2019, madrasLearningAdversariallyFair2018, ganin2016domain} aim at training models to obtain internal representations that are fair. The embeddings produced by these models cannot be used to predict the protected attribute $A$. Such works integrate an adversary with a new goal: trying to predict the protected attribute $A$ (and not degrading the model's performance anymore).

%Some approaches~\citep{raff2018, adel2019, madrasLearningAdversariallyFair2018, ganin2016domain, sattigeriFairnessGANGenerating2019} are inspired from adversarial machine learning but with the aim of predicting a protected attribute $A$ (e.g., gender or race) instead of degrading a model's performance.
%Some proposed methods reuse existing samples also to create fair models~\citep{raff2018, adel2019, madrasLearningAdversariallyFair2018, ganin2016domain, sattigeriFairnessGANGenerating2019}.
%They often use the existing training examples, with labels of a protected attribute $A$ (i.e. gender or race). 
%The adversary is in this case not tasked to trick the main model, but to predict the protected attribute $A$. 

%The adversary, that predicts the protected attribute $A$, can be integrated in the main model. 
%This gives us a model with two goals.
%Combining the initial model's goal with the one intended by the adversary,
A new model is created but with two goals:
(i) predicting the main attribute $Y$ (which we will refer to as the utility of the model);
(ii) not being able to predict the protected attribute $A$. 
They can be formally defined using minimax~\citep{edwards2015}: 

\begin{equation}
    \label{eq:minimax}
    \min_\theta \max_\phi L\left(\theta, \phi\right),
\end{equation}
%
with an adversary $\phi$ and an encoder with parameters $\theta$. 
%This minimax problem~\citep{edwards2015} is general, but we can restrict ourselves to a network that generates a hidden representation $R$ from the original input $X$. 
We use this representation to predict both $Y$ and $A$ via an adversarial network.
%This representation is used to predict the true target label $Y$, and by an adversarial network that tries to predict the protected attribute $A$. 
%This gives a loss function
\citet{ganin2016domain, raff2018, adel2019} all proposed to optimize a variant of the following loss function:

\begin{equation}
  \label{eq:loss}
  L(\theta, \phi) = E_{\theta, \phi}(X, Y) - \lambda D_{\theta, \phi}(X, A),
\end{equation}
%
with $D_{\theta, \phi}$ the loss for predicting $A$ from $X$, and $E_{\theta, \phi}$ the loss for the target prediction $Y$ also from $X$ and $\lambda$ a hyper-parameter.

\citet{zemel2013learning} learn \emph{fair representations} $X^*$ of the original input features $X$. 
%The idea is to remove possible dependencies that can exist between the representation and the protected attribute $A$ that an adversary could use to predict $A$. 
The idea is to remove existing dependencies between the representation $X$ and the protected attribute $A$, making its prediction impossible for adversaries.
This would make the practice of \emph{red-lining} also impossible, as these dependencies can no longer be correlated with $A$.
We consider this goal as a good proxy for fairness and this approach has been further investigated~\citep{raff2018, adel2019, madrasLearningAdversariallyFair2018}.

\subsection{Fairness through a Gradient Reversal Layer (GRL)}\label{ss:gradient_reversal}
%\citet{goodfellowGenerativeAdversarialNets2014a} addresses the minimax formulation by updating either the model's parameters $\theta$ or the adversary's parameters $\phi$.
\citet{ganin2016domain} introduced a \emph{gradient reversal layer} (GRL) originally for domain adaptation. 
Both \citet{raff2018} and \citet{adel2019} treated the protected attribute $A$ as a domain label.
The gradient reversal strategy assumes that multiplying by a negative sign will increase the loss of the branch $h_a: X \rightarrow \hat{A}$ and yields a representation $X^*$ that is maximally invariant to changes in $A$~\cite{adel2019, raff2018}. 
For a model with two target outputs and a hidden internal representation, Equation~\ref{eq:loss} applies. In our framework, the Reader (see \autoref{fig:architecture}) reuses this approach to mitigate the ability to predict $A$.

%However, \citet{ganin2016domain} made no guarantees as to how the domain was represented internally. 
%In this subsection, we argue that the adversarial branch achieves its goal by training the model specifically for predicting the protected attribute, not to be ignorant about it. 
%Intuitively, this makes sense, but there is no guarantee that gradient descent with flipped gradients does guarantee this maximal invariance.

\subsection{Adversarial attacks on model inputs}\label{ss:adv-attacks}

Our framework uses a second kind of adversarial machine learning, known as \emph{evasion attacks}~\citep{biggio2013evasion}, to diversify the training set.
The goal of the evasion attacks is to generate new examples that do not follow the same distribution as the original set. Generated examples combine different characteristics, initially under-represented. These examples can be added to the training set to perform adversarial retraining.
%By controlling the label assigned to these new examples and adding them to the training set, the learnt decision function should be modified accordingly.

%Algorithm~\ref{alg:evasion} reports the original algorithm given by \citet{biggio2013evasion}.
%%
%\begin{algorithm}
%\caption{The gradient-descent evasion attack proposed by~\citet{biggio2013evasion}}
%\label{alg:evasion}
%    \textbf{Input: } \textit{$x^0$}, the initial example; \textit{t}, the step size; \textit{$\lambda$}, the trade-off parameter; \textit{$\epsilon > %0$}, a small constant\\
%    \textbf{Output: }\textit{$x^{*}$}, the final attack point
%    \begin{algorithmic}
%        \STATE(1) m = 0;
%        \REPEAT
%            \STATE(2) m = m+1;
%            \STATE(3) Set $\nabla F(x^{m-1})$ to a unit vector aligned with $\nabla g(x^{m-1}) - \lambda \nabla p(x^{m-1} \vert y^c = -1)$;
%            \STATE(4) $x^m$ = $x^{m-1} - t\nabla F(x^{m-1})$;
%            \IF{ d($x^m,x^0$) $> d_{max}$}
%                \STATE(5) Project $x^m$ onto the boundary of the feasible region;
%            \ENDIF
%        \UNTIL{$F(x^{m}) - F(x^{m-1}) < \epsilon$}
%        \STATE(6) return $x^{*}$ = $x^m$;
%    \end{algorithmic}
%\end{algorithm}
%
%$x^0$ represents an example that is known (for which the classifier have given an answer when probing it).
%Since the evasion attack is a gradient-based method, $t$ is the step size allowing the algorithm to converge towards a local optimum.
%$\lambda$ is a trade-off parameter to prevent marginally interesting changes (because it will follow the data distribution of the training set).
%$\epsilon$ is a stopping criterion, avoiding to spend computation time in near-flat gradient areas.
%The heart of the algorithm is statement (3).
%It computes the direction of the modifications to apply in the feature space according to the separating function of the model.
%The computation of $\nabla F(x^{m-1})$ ensures that the directions of the modifications are optimal towards the separating function, in the end, resulting in a new example that mixes both features from the original example and features that makes the classifier decides that the new example should belong to an other class.
%As explained in \citep{biggio2013evasion}, $g(x^{m-1})$ represents the discriminant function of a classifier (used to give a decision based on its sign) and it needs to be defined depending on the model to be attacked and their hyper-parameters.
Evasion attacks are a gradient-based method and use a step size parameter $t$ to converge towards a local optimum.
An attack: (i) chooses a starting example for which the classifier's decision is known; (ii) computes the gradient directed towards the separating functions; (iii) applies this direction to the example's position scaled by $t$; (iv) repeats until a stopping criterion is met (number of iterations or a plateau is reached).
This algorithm has been implemented and made publicly available in the Python secML package~\footnote{https://secml.gitlab.io/} that we will use in our experiments.

%An important point showed by Demontis et al~\citep{demontis2019transfer} is the transferability potential of such attacks.
\citet{demontis2019transfer} showed the transferability potential of such attacks. In particular, from the attacker's point of view, building the exact, same model is not necessary. Data distributions to train both models should be similar. Hence, one can approximate any complex or non-derivable ML models with simpler ones and still generate relevant examples to influence the original model while retraining. The Feeder of our framework aims at providing adversarial examples for retraining that will mitigate unfairness.

%But the distribution of the data used to train the surrogate should be close to the training set used for the target model, the algorithm used to build the model does not have to be the same.

%An attacker could want to attack a decision tree (which is not derivable preventing the computation of $\nabla F(x^{m-1}$ making it potentially robust to such kind of attacks) with an SVM.
%It is an important result since, nowadays, ML models tend to be extremely performant but also very complex making them difficult to reconstruct, however, this result suggests that we could approach the decision function with a different one (somewhat "sufficiently similar") and the attacks performed on this approximation would also be good candidates for the original model.

\subsection{Discrimination-Aware Data Mining}
In works on \emph{discrimination-aware data mining} (DADM) and fairness in machine learning,
modifications to the data, the learning algorithms, or the resulting patterns and models \citep{DBLP:journals/tkde/HajianD13} have been developed and applied.
%, in which we situate our contribution. 
\citet{pedreschi2008discrimination} 
%introduced an approach to tackle this by extracting classification rules and ranking them based on a measure of discrimination.
introduced an approach to tackle discrimination by extracting classification rules and ranking them based on a measure.
DADM focuses on \emph{discovering discrimination} 
%(exploratory DADM~\citep{berendt2014better, custers2013discrimination}) 
as well as \emph{preventing discrimination}, both  
%In both cases, the first step is the discovery, which can focus on 
direct or indirect discrimination, the latter is the reason why simply removing protected attributes is not effective (see \autoref{sec:intro}).
Our framework performs both steps in an integrated manner by generating new examples and tuning the model to prevent discrimination.
%Our framework performs the two steps in integrated manner by improving the representation in the data and tuning the model parameters to prevent discrimination. 



%This is related to our adversary and the adversarial machine learning presented in \autoref{ss:adv-ml}. 
%One particular difference is the integration, instead of a two-step approach.


==> critique-of-GRL.tex <==
\section{Why gradient reversal is not a silver bullet}
\label{ss:biases-in-grl}

%\bettinanote{I have an issue with the term ``biased representations'' here, and would like to avoid it if possible. I haven't purged it from the text though. Maybe we need one more iteration for defining it?}
%\subsection{Biases in unbiased representations}
%BB 2020-04-01: Transition
As described in Section \ref{ss:gradient_reversal}, GRL is a currently popular approach, also known as `adversarial fairness'. We also use this technique, and like the authors who used it to learn `fair(er) representations'~\citep{adel2019, raff2018}, we find that it can mitigate unfairness in classification/prediction tasks. 

%Second, adversarial learning via gradient reversal {\em may, but need not,} achieve its main goal:
%the removal of information about the protected attribute. The outcome may even be the opposite of this, as is illustrated later on in \autoref{fig:tsne-unbiased}.
%We found 
%In the remainder of this section, we formulate and prove this problem, and illustrate it on COMPAS in \autoref{fig:tsne}.
In the remainder of this section, we formulate and prove this problem and illustrate it in \autoref{fig:tsne}.

The introduction of a gradient reversal layer by \citet{ganin2016domain} targeted domain adaptation. \citet{adel2019, raff2018} continued on this by viewing the protected attribute $A$ as a domain label. 
However, \citet{ganin2016domain} offered no guarantees as to how the domain was represented internally. 
In this section, we argue that the adversarial branch achieves its goal by learning specifically to predict the protected attribute, %not to be ignorant about it. 
rather than obfuscating it.

The gradient reversal strategy assumes that multiplying by a negative sign will increase the loss of the branch $h_a: X \rightarrow \hat{A}$ that then yields a representation $X^*$ that is maximally invariant to changes in $A$~\cite{adel2019}. 
This is intuitive, but there is no guarantee that gradient descent with flipped gradients does guarantee this maximal invariance.

\begin{lemma}
  \label{lemma:grad}
  Gradient reversal equates to perform gradient ascent on the shared layers with respect to the protected attribute $A$, 
  whilst simultaneously performing gradient descent on the dedicated branch for the attribute $A$.
\end{lemma}

\begin{proof}
  Consider the final layer $L$ with two independent branches, governed by parameters $\theta$ and $\phi$ respectively, and the shared penultimate layer $L-1$. The shared loss function for both is stated earlier in \autoref{eq:loss}. For the branch that predicts the protected attribute $A$, the loss $D_{\theta,\phi}^{'} (X, A)$ gives rise to the weight updates $\Delta w_{\phi}^{(L)}$ for the weights of the branch $h_a: X \rightarrow \hat{A}$, following     

  \begin{equation}
    \Delta w_{\phi}^{(L)} = - \alpha \lambda \frac{\partial D_{\theta,\phi} }{ \partial w_{\phi}^{(L)} }.
  \end{equation}

  %The other branch for the target label $Y$ is updated in a similar way.
  The branch giving target label $Y$ is updated similarly. The shared penultimate layer's weights rely on the shared loss $L(\theta, \phi)$ and are updated following 

  \begin{equation}
    \Delta w^{(L-1)} = - \alpha \frac{\partial E_{\theta, \phi} }{ \partial w^{(L-1)} } + \alpha \lambda \frac{ \partial D_{\theta, \phi}}{ \partial w^{(L-1)} }
    .
  \end{equation}
  
  %%\bettinanote{embarrassing Q that shows once more I need to read up on neural networks ...: if this is with respect to equation 2, why is it always $\alpha$ and neither $\beta$ nor $\gamma$?}
  %% Adjusted the referred equation as it was a different alpha ...
  %So with respect to the loss $D_{\theta,\phi} (X, A)$, the weights $w_{\phi}^{(L)}$ are updated following gradient descent, thus minimizing the loss for this branch. 
  The weights $w_{\phi}^{(L)}$ are updated following gradient descent with respect to the loss $D_{\theta,\phi} (X, A)$, thus minimizing the loss for this branch.
  However, gradient reversal simultaneously performs gradient ascent with respect to the same loss $D_{\theta,\phi} (X, A)$ on all weights of layers $1, \dots, L - 1$. The shared layers still perform gradient descent with regard to the loss $E_{\theta, \phi}(X, Y) $ for the target label $Y$.
 
  %\qed
\end{proof}

We have shown that 
the % BB 2020-04-01
shared penultimate layer does not perform gradient descent, but % it does perform BB 2020-04-01 
gradient ascent. This is in accordance with the implicit definition for maximal variance~\citep{adel2019, ganin2016domain, raff2018} following 

  \begin{equation}
    \max_\phi D_{\theta,\phi} (X, A).
\end{equation}

This fits in the larger minimax problem from \autoref{eq:minimax} and results in a saddle point~\citep{ganin2016domain}. However, the end result is not guaranteed to be a maximal invariant representation. 
In the worst case, maximizing this loss $D_{\theta,\phi} (X, A)$ can even result in the opposite optimum for the shared trunk with regard to $A$. This means that the model is not necessarily maximally invariant on $(L-1)$. We need to emphasize that this is a {\em theoretical} result, but it calls for caution when adversarial fairness is to be used to, for example, publish or re-use a supposedly `fair' data representation. We illustrate this issue on the COMPAS dataset in \autoref{fig:tsne}.

\begin{figure}[tbh]
  \centering
  \centerfloat
  \begin{subfigure}[t]{0.3\columnwidth}
    \includegraphics[width=\columnwidth]{fig/tsne_biased_small.png}
    \caption{Naive model}
    \label{fig:tsne-biased}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\columnwidth}
    \includegraphics[width=\columnwidth]{fig/tsne_debiased_small.png}
    \caption{Model trained with a GRL ($\lambda=50$)}
    \label{fig:tsne-unbiased}
  \end{subfigure}
    ~
  \begin{subfigure}[t]{0.3\columnwidth}
    \includegraphics[width=\columnwidth]{fig/tsne_debiased_ours}
    \caption{Model trained with our framework}
    \label{fig:tsne-unbiased-ours}
  \end{subfigure}
  \caption{T-SNE dimensionality reduction of the activations in the last hidden layer on the held-out COMPAS test set. Distinct colors are used for the reported race of individuals in the dataset: either African-American \statcirc{paper_blue} or Caucasian \statcirc{paper_orange}.}\label{fig:tsne}
\end{figure}


For each individual for the COMPAS test set, all three models derive a representation in the last hidden layer, on which
we applied a t-SNE dimensionality reduction for a two-dimensional visualisation.
%The protected attribute $A$, \emph{i.e.} race, is also shown for these individuals.

The model without fairness constraints (\autoref{fig:tsne-biased}) has slight separation with regard to the protected attribute, 
but it is clearly separable in the representation from the model trained with a GRL (\autoref{fig:tsne-unbiased}).
This is also shown by retraining a one-layer perceptron on these representation. The model that was originally trained to predict only recidivism could be used to classify the protected attribute race with $AUC=0.71$. And although the original GRL reported an $AUC=0.44$, \autoref{lemma:grad} tells us that this adversary cannot be trusted. Which is the case here, as an independent perceptron has $AUC=0.92$. \citet{elazar-goldberg-2018-adversarial} made an empirical observation on \emph{leakage} of protected attributes specifically for text-based classifiers that can also be traced back to this.

%The figures show that a model trained with a GRL (\autoref{fig:tsne-unbiased}) can have more biased representations in the last hidden layer than a naive model (\emph{i.e.} without fairness constraints, \autoref{fig:tsne-biased}).
%However, gradient reversal is only {\em one} component of our architecture. 
Here, we demonstrated that the hidden representation obtained by gradient reversal, not only still contains information about the protected attribute, but contains a stronger signal. Our architecture that joins `adversarial fairness' and `adversarial learning' (see Section \ref{ss:motivating-scenarios} and Fig. \ref{fig:architecture}) leverages utility- {\em and} fairness-focused methods in a better way than the modification of the model alone. By injecting noise with the adversarial Feeder, our framework makes the protected attribute $A$ a useless predictor, as shown in \autoref{fig:tsne-unbiased-ours}.
Our results, discussed in Section \ref{ss:results}, confirm this expectation. 
 
%Thus, these representations can serve as an even better predictor.
 %the Feeder introduces examples that  make  the protected attribute $A$ a useless predictor.
%Note that T-SNE is mainly for visualization purposes and based on a stochastic process.




==> introduction.tex <==
%\subsection{Context}
%The proliferation of machine learning allows various actors to easily deploy systems that classify people based on some data those actors collected; and this classification can have a real effect on people.
Machine learning eases the deployment of systems that tackles various tasks: spam filtering, image recognition, gesture recognition, etc.
One of the most trendy applications is decision support. After collecting data on people and their context, these systems give recommendations on who should get a loan, predict who may commit subsequent offences, etc. However, this support can have detrimental consequences.
Well-studied examples include the COMPAS system that predicts the recidivism of pre-trial inmates~\citep{angwinMachineBiasThere2016, chouldechovaFairPredictionDisparate2017} or accepting credit applications, or more recently the issues with Apple's credit card that resulted in vastly lower spending limits for women. Such systems may amplify the prevalent situation by imposing more expensive loans to African-American people, who then fail to repay them more often~\citep{overdorfQuestioningAssumptionsFairness2018, ensign2017}. These ``positive" feedback loops should be detected and mitigated.  

Training a machine learning model can be costly, is sensitive to the data quality, and may result in a complex model. Hence, the decision process may fail to be transparent, which ushers in discrimination or unfair treatment for protected groups. But how to perform this assessment when decisions are often neither interpretable nor intuitive?
Researchers have focused on providing quantitative assessments (\emph{e.g.} demographic parity~\citep{dworkFairnessAwareness2012}, equalized odds~\citep{hardtEqualityOpportunitySupervised2016}, statistical parity~\citep{feldman2015certifying, zemel2013learning}, disparate impact~\citep{chouldechovaFairPredictionDisparate2017,feldman2015certifying},
% BB 2020-04-03: I added Feldman et al.
Darlington criterion~\citep{darlington1971}, threshold testing~\citep{pmlr-v84-pierson18a}) all covering a specific fairness aspect.
%Are these systems fair?
%Since these decisions are often made in a way that is neither interpretable or intuitive, this question resulted in many researchers presenting their own metric for fairness, \emph{e.g.} demographic parity, group fairness, statistical parity, predictive parity, Darlington criterion, etc.~\citep{hardtEqualityOpportunitySupervised2016, angwinMachineBiasThere2016, chouldechovaFairPredictionDisparate2017, corbett-davies2017, feldman2015certifying, darlington1971}.  

%Most of this research constructs the issue as a statistical problem with the protected attribute $A$ being a random variable, where there are dependencies between this protected attribute (race, gender, \dots) and other attributes (ZIP code, occupation, \dots). 
%These dependencies are the heart of why only removing the protected attribute, sometimes referred to as \emph{fairness through unawareness}, is well-known as an insufficient approach to mitigate biases~\citep{pedreshi2008discrimination}.
To tackle this problem, researchers assume that a protected attribute $A$ (\emph{e.g.}, race or gender) exists while it should not be predictable, despite existing dependencies between this attribute and others (ZIP code, \dots). Thus, only removing the protected attribute, sometimes referred to as \emph{fairness through unawareness}, is known to be insufficient~\citep{pedreschi2008discrimination, calders2013unbiased}. 
%This is because people and machine learning-based systems can still use these dependencies (\emph{e.g.} ZIP code) to target protected groups---either intentionally or not---which is a concept known as \emph{redlining}.

Because of the far-reaching consequences---being encoded in legal obligations---of these machine learning systems, state-of-the-art methods employ more advanced approaches to mitigate unfairness issues with these models inspired by other machine learning domains, like domain adaptation. One technique is not enough to harness this complex problem. Here, we propose to use two kinds of adversarial machine learning techniques, which we motivate through the following scenarios.
%One of these methods is to introduce an adversary that tries to recognize $A$.
%The system is then optimized such that the performance of this adversary is no better than random.
%This approach, called \emph{adversarial fairness}, has been applied for autoencoders~\citep{louizosVariationalFairAutoencoder2015, edwards2015, madrasLearningAdversariallyFair2018} and for both classification and regression networks~\citep{zhangMitigatingUnwantedBiases2018, raff2018, adel2019, sattigeriFairnessGANGenerating2019, liuIncorporatingPriorsFeature2019}.

\subsection{Motivating Scenarios}
\label{ss:motivating-scenarios}

Our goal is to develop a notion of \textit{ethical adversaries} based on adversarial machine learning techniques, initially designed to fool machine learning classifiers, to improve their fairness. Our scenarios take place in the context of an ethics assessment activity while designing a new machine learning-based system for a fictional company called ``Fancy-Fair AI". 

\textit{The Feeder: Black-box External Attacks.}
Alice is a specialist in adversarial machine learning (advML) attacks. 
%She masters the many ways of fooling machine learning classifiers by generating instances in areas of low confidence.  
She is hired for a mission at Fancy-Fair AI to assess and improve the dataset to increase the performance of the trained machine learning model, later on.
However, she is only given the dataset and not the inner details of the already trained black-box machine learning model. Therefore, she has to train a surrogate classifier on the dataset and will feed the machine learning model with new instances. 
%In particular, she generates new instances via \textit{evasion attacks} as proposed by Biggio et al. \citep{biggio2013evasion}. 
This process, known as \textit{evasion attacks} \citep{biggio2013evasion}, starts from an existing instance and create a new one by modifying feature values along the gradient in yet unseen zones of the feature space (\textit{i.e.}, where the prediction confidence is low) through successive displacements. Alice ensures the validity of modified features and tunes the attacks' parameters to improve the system via retraining. Alice crafts examples that are also black-box for fairness evaluation as they are not tuned to optimise a particular metric. Yet, such examples can help the Reader to alleviate misrepresentations as they will provide new feature value combinations. 

\textit{The Reader: White-box Adversarial Fairness.}
Bob is an ethics assessment officer at Fancy-Fair AI. He leans on a set of carefully selected fairness metrics assuming that fair decisions should not depend on some protected attributes (race, gender, etc.). Therefore Bob wants to ensure that an insider adversary, striving to predict the value of a protected attribute (e.g., gender) given an outcome (\emph{e.g.}, credit limit), fails to do so. This approach, called \emph{adversarial fairness}, has been applied for autoencoders~\citep{louizosVariationalFairAutoencoder2015, edwards2015, madrasLearningAdversariallyFair2018} and for both classification and regression networks~\citep{zhangMitigatingUnwantedBiases2018, raff2018, adel2019}. 
It relies on a \textit{gradient reversal} \citep{ganin2016domain} to update the weights of the adversary so that the chance of predicting the protected attribute is no better than random. This relies on diminishing the dependencies between the protected attribute and the other attributes by backpropagating the gradients with gradient ascent.

%This relies on creating a fair representation by backpropagating the gradients to remove every predictive feature, which is the opposite of normal gradient descent.

%Bob, then, tunes the parameters of the system accordingly to his results with the conviction that the adversary cannot rely on a machine learning model to predict the protected attribute anymore.
%Bob then tunes the parameters of the system so that the performance of the the adversary is no better than random. 

%Bob integrates this adversary in the training of the ML algorithm and achieves a certain level of fairness. %While Bob is happy with his current technique, he wonders how fairness may evolve with respect to the (mis)representation of certain categories.

%\gillesnote{moved the paragraph from the context to here:}

%Because of the far-reaching consequences---which are also encoded in legal obligations---of these machine learning systems, state-of-the-art methods employ more advanced approaches to mitigate or remove biases from these models. One of these methods is to introduce an adversary that's tasked to recognize this protected attribute. The system is then optimized that the performance of this adversary is no better than random. This approach, called \emph{adversarial fairness}, has been applied for autoencoders~\citep{louizosVariationalFairAutoencoder2015, edwards2015, madrasLearningAdversariallyFair2018} and for both classification and regression networks~\citep{zhangMitigatingUnwantedBiases2018, raff2018, adel2019, sattigeriFairnessGANGenerating2019, liuIncorporatingPriorsFeature2019}. 

\textit{Feed, Read and Fix: Grey-box Fairness.}
This last scenario, which illustrates the main contribution of this paper, reunites Alice and Bob approaches as depicted in \autoref{fig:architecture}. This integrated architecture thus works both at the data level (by providing new instances) and at the model level (by preventing it from guessing protected attributes). Fancy-Fair AI monitors the effectiveness of the integrated solution by monitoring demographic parity and equal opportunity and the impact on the utility (accuracy, F${_1}$) of the decision system.

\begin{figure}[tbh]
  \centering
  \includegraphics[width=0.85\textwidth]{fig/architecture_detailed_trimmed}
  \caption{Our ethical adversaries framework: the feeder (Alice) improves the target Y by creating new instances X, while the reader (Bob) prevents from guessing A. The modified prediction due to model adaptation is shown bottom-right.}
  \label{fig:architecture}
\end{figure}



%Fancy-Fair AI wants that the construction of the ML decisions includes fairness considerations by preventing from an ethical adversary to guess protected attributes and to alleviate (mis)representation of certain categories in the dataset by generating realistic cases in areas of the feature space where the ML algorithm is less confident. Alice and Bob work hand-in-hand with their ethical adversaries to improve fairness from the model and data perspectives. This scenario integration is depicted Figure \ref{fig:architecture}.
%In this figure, Scenario \#1 is represented by the upper box between the system and the adversarial attack side, while the second scenario is represented by the right side of the figure.

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=\textwidth]{figure_fairness.png}
%    \caption{An integrated adversarial scenario to improve fairness}
%    \label{fig:big_pic}
%\end{figure}


\subsection{Contributions and Organisation}

In this paper, we propose a new framework implementing the grey-box fairness scenario. We make the following contributions:
\begin{itemize}
    \item The definition of the behaviour of our ethical adversaries in terms of evasion attacks and gradient reversal analyses;
    \item Demonstration of an undesired side-effect of gradient-based fairness models;
    \item An implementation of our framework in Python\footnote{Available at {\tt http://<url removed for double blind review>}};
    \item Evaluation on three datasets: COMPAS, German Credit and Adult; showing state-of-the-art level results in demographic parity and equal opportunity metrics while globally improving the model's utility. 
\end{itemize}

%We provide with a new solution that brings together evasion adversarial attacks proposed by Biggio et al. \citep{biggio2013evasion} and \emph{adversarial fairness} both for mitigating biases via adversarial retraining, that provides new examples outside the initial data distribution, and to counter the prediction of protected attributes.

This paper is organised as follows: \autoref{sec:background} discusses 
related work on adversarial machine learning techniques as well as %other work trying to evaluate fairness.
on measuring and mitigating unfairness.
% BB 2020-04-02: sentence is not great, but I can't think of a better one right now.
\autoref{ss:biases-in-grl} investigates a problem of gradient reversal methods.
\autoref{sec:our-work} presents %, in detail, 
our new framework, followed by its evaluation on the COMPAS, German Credit and Adult datasets in \autoref{sec:evaluation}. \autoref{sec:conclusion} concludes and gives an outlook on future work.

%\subsection{Paper Organisation}

